Signaling Game-based Misbehavior Inspection in V2I-enabled Highway Operations

Vehicle-to-Infrastructure (V2I) communications are increasingly supporting highway operations such as electronic toll collection, carpooling, and vehicle platooning. In this paper we study the incentives of strategic misbehavior by individual vehicles who can exploit the security vulnerabilities in V2I communications and negatively impact the highway operations. We consider a V2I-enabled highway segment facing two classes of vehicles (agent populations), each with an authorized access to one server (subset of lanes). Vehicles are strategic in that they can misreport their class (type) to the system operator and get an unauthorized access to the server dedicated to the other class. This misbehavior causes additional congestion externality on the compliant vehicles, and thus, needs to be deterred. We focus on an environment where the operator is able to inspect the vehicles for misbehavior. The inspection is costly and successful detection incurs a fine on the misbehaving vehicle. We formulate a signaling game to study the strategic interaction between the vehicle classes and the operator. Our equilibrium analysis provides conditions on the cost parameters that govern the vehicles' incentive to misbehave or not. We also determine the operator's equilibrium inspection strategy.

==> colordef.tex <==
\definecolor{snow}{rgb}{1.000,0.980,0.980}
\definecolor{snow1}{rgb}{1.000,0.980,0.980}
\definecolor{snow2}{rgb}{0.933,0.914,0.914}
\definecolor{snow3}{rgb}{0.804,0.788,0.788}
\definecolor{snow4}{rgb}{0.545,0.537,0.537}
\definecolor{GhostWhite}{rgb}{0.973,0.973,1.000}
\definecolor{WhiteSmoke}{rgb}{0.961,0.961,0.961}
\definecolor{gainsboro}{rgb}{0.863,0.863,0.863}
\definecolor{FloralWhite}{rgb}{1.000,0.980,0.941}
\definecolor{OldLace}{rgb}{0.992,0.961,0.902}
\definecolor{linen}{rgb}{0.980,0.941,0.902}
\definecolor{AntiqueWhite}{rgb}{0.980,0.922,0.843}
\definecolor{PapayaWhip}{rgb}{1.000,0.937,0.835}
\definecolor{BlanchedAlmond}{rgb}{1.000,0.922,0.804}
\definecolor{bisque}{rgb}{1.000,0.894,0.769}
\definecolor{PeachPuff}{rgb}{1.000,0.855,0.725}
\definecolor{NavajoWhite}{rgb}{1.000,0.871,0.678}
\definecolor{moccasin}{rgb}{1.000,0.894,0.710}
\definecolor{cornsilk}{rgb}{1.000,0.973,0.863}
\definecolor{ivory}{rgb}{1.000,1.000,0.941}
\definecolor{LemonChiffon}{rgb}{1.000,0.980,0.804}
\definecolor{seashell}{rgb}{1.000,0.961,0.933}
\definecolor{honeydew}{rgb}{0.941,1.000,0.941}
\definecolor{MintCream}{rgb}{0.961,1.000,0.980}
\definecolor{azure}{rgb}{0.941,1.000,1.000}
\definecolor{AliceBlue}{rgb}{0.941,0.973,1.000}
\definecolor{lavender}{rgb}{0.902,0.902,0.980}
\definecolor{LavenderBlush}{rgb}{1.000,0.941,0.961}
\definecolor{MistyRose}{rgb}{1.000,0.894,0.882}
\definecolor{white}{rgb}{1.000,1.000,1.000}
\definecolor{black}{rgb}{0.000,0.000,0.000}
\definecolor{DarkSlateGray}{rgb}{0.184,0.310,0.310}
\definecolor{DimGray}{rgb}{0.412,0.412,0.412}
\definecolor{SlateGray}{rgb}{0.439,0.502,0.565}
\definecolor{LightSlateGray}{rgb}{0.467,0.533,0.600}
\definecolor{gray}{rgb}{0.745,0.745,0.745}
\definecolor{LightGray}{rgb}{0.827,0.827,0.827}
\definecolor{MidnightBlue}{rgb}{0.098,0.098,0.439}
\definecolor{navy}{rgb}{0.000,0.000,0.502}
\definecolor{NavyBlue}{rgb}{0.000,0.000,0.502}
\definecolor{CornflowerBlue}{rgb}{0.392,0.584,0.929}
\definecolor{DarkSlateBlue}{rgb}{0.282,0.239,0.545}
\definecolor{SlateBlue}{rgb}{0.416,0.353,0.804}
\definecolor{MediumSlateBlue}{rgb}{0.482,0.408,0.933}
\definecolor{LightSlateBlue}{rgb}{0.518,0.439,1.000}
\definecolor{MediumBlue}{rgb}{0.000,0.000,0.804}
\definecolor{RoyalBlue}{rgb}{0.255,0.412,0.882}
\definecolor{blue}{rgb}{0.000,0.000,1.000}
\definecolor{DodgerBlue}{rgb}{0.118,0.565,1.000}
\definecolor{DeepSkyBlue}{rgb}{0.000,0.749,1.000}
\definecolor{SkyBlue}{rgb}{0.529,0.808,0.922}
\definecolor{LightSkyBlue}{rgb}{0.529,0.808,0.980}
\definecolor{SteelBlue}{rgb}{0.275,0.510,0.706}
\definecolor{LightSteelBlue}{rgb}{0.690,0.769,0.871}
\definecolor{LightBlue}{rgb}{0.678,0.847,0.902}
\definecolor{PowderBlue}{rgb}{0.690,0.878,0.902}
\definecolor{PaleTurquoise}{rgb}{0.686,0.933,0.933}
\definecolor{DarkTurquoise}{rgb}{0.000,0.808,0.820}
\definecolor{MediumTurquoise}{rgb}{0.282,0.820,0.800}
\definecolor{turquoise}{rgb}{0.251,0.878,0.816}
\definecolor{cyan}{rgb}{0.000,1.000,1.000}
\definecolor{LightCyan}{rgb}{0.878,1.000,1.000}
\definecolor{CadetBlue}{rgb}{0.373,0.620,0.627}
\definecolor{MediumAquamarine}{rgb}{0.400,0.804,0.667}
\definecolor{aquamarine}{rgb}{0.498,1.000,0.831}
\definecolor{DarkGreen}{rgb}{0.000,0.392,0.000}
\definecolor{DarkOliveGreen}{rgb}{0.333,0.420,0.184}
\definecolor{DarkSeaGreen}{rgb}{0.561,0.737,0.561}
\definecolor{SeaGreen}{rgb}{0.180,0.545,0.341}
\definecolor{MediumSeaGreen}{rgb}{0.235,0.702,0.443}
\definecolor{LightSeaGreen}{rgb}{0.125,0.698,0.667}
\definecolor{PaleGreen}{rgb}{0.596,0.984,0.596}
\definecolor{SpringGreen}{rgb}{0.000,1.000,0.498}
\definecolor{LawnGreen}{rgb}{0.486,0.988,0.000}
\definecolor{green}{rgb}{0.000,1.000,0.000}
\definecolor{chartreuse}{rgb}{0.498,1.000,0.000}
\definecolor{MediumSpringGreen}{rgb}{0.000,0.980,0.604}
\definecolor{GreenYellow}{rgb}{0.678,1.000,0.184}
\definecolor{LimeGreen}{rgb}{0.196,0.804,0.196}
\definecolor{YellowGreen}{rgb}{0.604,0.804,0.196}
\definecolor{ForestGreen}{rgb}{0.133,0.545,0.133}
\definecolor{OliveDrab}{rgb}{0.420,0.557,0.137}
\definecolor{DarkKhaki}{rgb}{0.741,0.718,0.420}
\definecolor{khaki}{rgb}{0.941,0.902,0.549}
\definecolor{PaleGoldenrod}{rgb}{0.933,0.910,0.667}
\definecolor{LightGoldenrodYellow}{rgb}{0.980,0.980,0.824}
\definecolor{LightYellow}{rgb}{1.000,1.000,0.878}
\definecolor{yellow}{rgb}{1.000,1.000,0.000}
\definecolor{gold}{rgb}{1.000,0.843,0.000}
\definecolor{LightGoldenrod}{rgb}{0.933,0.867,0.510}
\definecolor{goldenrod}{rgb}{0.855,0.647,0.125}
\definecolor{DarkGoldenrod}{rgb}{0.722,0.525,0.043}
\definecolor{RosyBrown}{rgb}{0.737,0.561,0.561}
\definecolor{IndianRed}{rgb}{0.804,0.361,0.361}
\definecolor{SaddleBrown}{rgb}{0.545,0.271,0.075}
\definecolor{sienna}{rgb}{0.627,0.322,0.176}
\definecolor{peru}{rgb}{0.804,0.522,0.247}
\definecolor{burlywood}{rgb}{0.871,0.722,0.529}
\definecolor{beige}{rgb}{0.961,0.961,0.863}
\definecolor{wheat}{rgb}{0.961,0.871,0.702}
\definecolor{SandyBrown}{rgb}{0.957,0.643,0.376}
\definecolor{tan}{rgb}{0.824,0.706,0.549}
\definecolor{chocolate}{rgb}{0.824,0.412,0.118}
\definecolor{firebrick}{rgb}{0.698,0.133,0.133}
\definecolor{brown}{rgb}{0.647,0.165,0.165}
\definecolor{DarkSalmon}{rgb}{0.914,0.588,0.478}
\definecolor{salmon}{rgb}{0.980,0.502,0.447}
\definecolor{LightSalmon}{rgb}{1.000,0.627,0.478}
\definecolor{orange}{rgb}{1.000,0.647,0.000}
\definecolor{DarkOrange}{rgb}{1.000,0.549,0.000}
\definecolor{coral}{rgb}{1.000,0.498,0.314}
\definecolor{LightCoral}{rgb}{0.941,0.502,0.502}
\definecolor{tomato}{rgb}{1.000,0.388,0.278}
\definecolor{OrangeRed}{rgb}{1.000,0.271,0.000}
\definecolor{red}{rgb}{1.000,0.000,0.000}
\definecolor{HotPink}{rgb}{1.000,0.412,0.706}
\definecolor{DeepPink}{rgb}{1.000,0.078,0.576}
\definecolor{pink}{rgb}{1.000,0.753,0.796}
\definecolor{LightPink}{rgb}{1.000,0.714,0.757}
\definecolor{PaleVioletRed}{rgb}{0.859,0.439,0.576}
\definecolor{maroon}{rgb}{0.690,0.188,0.376}
\definecolor{MediumVioletRed}{rgb}{0.780,0.082,0.522}
\definecolor{VioletRed}{rgb}{0.816,0.125,0.565}
\definecolor{magenta}{rgb}{1.000,0.000,1.000}
\definecolor{violet}{rgb}{0.933,0.510,0.933}
\definecolor{plum}{rgb}{0.867,0.627,0.867}
\definecolor{orchid}{rgb}{0.855,0.439,0.839}
\definecolor{MediumOrchid}{rgb}{0.729,0.333,0.827}
\definecolor{DarkOrchid}{rgb}{0.600,0.196,0.800}
\definecolor{DarkViolet}{rgb}{0.580,0.000,0.827}
\definecolor{BlueViolet}{rgb}{0.541,0.169,0.886}
\definecolor{purple}{rgb}{0.627,0.125,0.941}
\definecolor{MediumPurple}{rgb}{0.576,0.439,0.859}
\definecolor{thistle}{rgb}{0.847,0.749,0.847}
\definecolor{seashell1}{rgb}{1.000,0.961,0.933}
\definecolor{seashell2}{rgb}{0.933,0.898,0.871}
\definecolor{seashell3}{rgb}{0.804,0.773,0.749}
\definecolor{seashell4}{rgb}{0.545,0.525,0.510}
\definecolor{AntiqueWhite1}{rgb}{1.000,0.937,0.859}
\definecolor{AntiqueWhite2}{rgb}{0.933,0.875,0.800}
\definecolor{AntiqueWhite3}{rgb}{0.804,0.753,0.690}
\definecolor{AntiqueWhite4}{rgb}{0.545,0.514,0.471}
\definecolor{bisque1}{rgb}{1.000,0.894,0.769}
\definecolor{bisque2}{rgb}{0.933,0.835,0.718}
\definecolor{bisque3}{rgb}{0.804,0.718,0.620}
\definecolor{bisque4}{rgb}{0.545,0.490,0.420}
\definecolor{PeachPuff1}{rgb}{1.000,0.855,0.725}
\definecolor{PeachPuff2}{rgb}{0.933,0.796,0.678}
\definecolor{PeachPuff3}{rgb}{0.804,0.686,0.584}
\definecolor{PeachPuff4}{rgb}{0.545,0.467,0.396}
\definecolor{NavajoWhite1}{rgb}{1.000,0.871,0.678}
\definecolor{NavajoWhite2}{rgb}{0.933,0.812,0.631}
\definecolor{NavajoWhite3}{rgb}{0.804,0.702,0.545}
\definecolor{NavajoWhite4}{rgb}{0.545,0.475,0.369}
\definecolor{LemonChiffon1}{rgb}{1.000,0.980,0.804}
\definecolor{LemonChiffon2}{rgb}{0.933,0.914,0.749}
\definecolor{LemonChiffon3}{rgb}{0.804,0.788,0.647}
\definecolor{LemonChiffon4}{rgb}{0.545,0.537,0.439}
\definecolor{cornsilk1}{rgb}{1.000,0.973,0.863}
\definecolor{cornsilk2}{rgb}{0.933,0.910,0.804}
\definecolor{cornsilk3}{rgb}{0.804,0.784,0.694}
\definecolor{cornsilk4}{rgb}{0.545,0.533,0.471}
\definecolor{ivory1}{rgb}{1.000,1.000,0.941}
\definecolor{ivory2}{rgb}{0.933,0.933,0.878}
\definecolor{ivory3}{rgb}{0.804,0.804,0.757}
\definecolor{ivory4}{rgb}{0.545,0.545,0.514}
\definecolor{honeydew1}{rgb}{0.941,1.000,0.941}
\definecolor{honeydew2}{rgb}{0.878,0.933,0.878}
\definecolor{honeydew3}{rgb}{0.757,0.804,0.757}
\definecolor{honeydew4}{rgb}{0.514,0.545,0.514}
\definecolor{LavenderBlush1}{rgb}{1.000,0.941,0.961}
\definecolor{LavenderBlush2}{rgb}{0.933,0.878,0.898}
\definecolor{LavenderBlush3}{rgb}{0.804,0.757,0.773}
\definecolor{LavenderBlush4}{rgb}{0.545,0.514,0.525}
\definecolor{MistyRose1}{rgb}{1.000,0.894,0.882}
\definecolor{MistyRose2}{rgb}{0.933,0.835,0.824}
\definecolor{MistyRose3}{rgb}{0.804,0.718,0.710}
\definecolor{MistyRose4}{rgb}{0.545,0.490,0.482}
\definecolor{azure1}{rgb}{0.941,1.000,1.000}
\definecolor{azure2}{rgb}{0.878,0.933,0.933}
\definecolor{azure3}{rgb}{0.757,0.804,0.804}
\definecolor{azure4}{rgb}{0.514,0.545,0.545}
\definecolor{SlateBlue1}{rgb}{0.514,0.435,1.000}
\definecolor{SlateBlue2}{rgb}{0.478,0.404,0.933}
\definecolor{SlateBlue3}{rgb}{0.412,0.349,0.804}
\definecolor{SlateBlue4}{rgb}{0.278,0.235,0.545}
\definecolor{RoyalBlue1}{rgb}{0.282,0.463,1.000}
\definecolor{RoyalBlue2}{rgb}{0.263,0.431,0.933}
\definecolor{RoyalBlue3}{rgb}{0.227,0.373,0.804}
\definecolor{RoyalBlue4}{rgb}{0.153,0.251,0.545}
\definecolor{blue1}{rgb}{0.000,0.000,1.000}
\definecolor{blue2}{rgb}{0.000,0.000,0.933}
\definecolor{blue3}{rgb}{0.000,0.000,0.804}
\definecolor{blue4}{rgb}{0.000,0.000,0.545}
\definecolor{DodgerBlue1}{rgb}{0.118,0.565,1.000}
\definecolor{DodgerBlue2}{rgb}{0.110,0.525,0.933}
\definecolor{DodgerBlue3}{rgb}{0.094,0.455,0.804}
\definecolor{DodgerBlue4}{rgb}{0.063,0.306,0.545}
\definecolor{SteelBlue1}{rgb}{0.388,0.722,1.000}
\definecolor{SteelBlue2}{rgb}{0.361,0.675,0.933}
\definecolor{SteelBlue3}{rgb}{0.310,0.580,0.804}
\definecolor{SteelBlue4}{rgb}{0.212,0.392,0.545}
\definecolor{DeepSkyBlue1}{rgb}{0.000,0.749,1.000}
\definecolor{DeepSkyBlue2}{rgb}{0.000,0.698,0.933}
\definecolor{DeepSkyBlue3}{rgb}{0.000,0.604,0.804}
\definecolor{DeepSkyBlue4}{rgb}{0.000,0.408,0.545}
\definecolor{SkyBlue1}{rgb}{0.529,0.808,1.000}
\definecolor{SkyBlue2}{rgb}{0.494,0.753,0.933}
\definecolor{SkyBlue3}{rgb}{0.424,0.651,0.804}
\definecolor{SkyBlue4}{rgb}{0.290,0.439,0.545}
\definecolor{LightSkyBlue1}{rgb}{0.690,0.886,1.000}
\definecolor{LightSkyBlue2}{rgb}{0.643,0.827,0.933}
\definecolor{LightSkyBlue3}{rgb}{0.553,0.714,0.804}
\definecolor{LightSkyBlue4}{rgb}{0.376,0.482,0.545}
\definecolor{SlateGray1}{rgb}{0.776,0.886,1.000}
\definecolor{SlateGray2}{rgb}{0.725,0.827,0.933}
\definecolor{SlateGray3}{rgb}{0.624,0.714,0.804}
\definecolor{SlateGray4}{rgb}{0.424,0.482,0.545}
\definecolor{LightSteelBlue1}{rgb}{0.792,0.882,1.000}
\definecolor{LightSteelBlue2}{rgb}{0.737,0.824,0.933}
\definecolor{LightSteelBlue3}{rgb}{0.635,0.710,0.804}
\definecolor{LightSteelBlue4}{rgb}{0.431,0.482,0.545}
\definecolor{LightBlue1}{rgb}{0.749,0.937,1.000}
\definecolor{LightBlue2}{rgb}{0.698,0.875,0.933}
\definecolor{LightBlue3}{rgb}{0.604,0.753,0.804}
\definecolor{LightBlue4}{rgb}{0.408,0.514,0.545}
\definecolor{LightCyan1}{rgb}{0.878,1.000,1.000}
\definecolor{LightCyan2}{rgb}{0.820,0.933,0.933}
\definecolor{LightCyan3}{rgb}{0.706,0.804,0.804}
\definecolor{LightCyan4}{rgb}{0.478,0.545,0.545}
\definecolor{PaleTurquoise1}{rgb}{0.733,1.000,1.000}
\definecolor{PaleTurquoise2}{rgb}{0.682,0.933,0.933}
\definecolor{PaleTurquoise3}{rgb}{0.588,0.804,0.804}
\definecolor{PaleTurquoise4}{rgb}{0.400,0.545,0.545}
\definecolor{CadetBlue1}{rgb}{0.596,0.961,1.000}
\definecolor{CadetBlue2}{rgb}{0.557,0.898,0.933}
\definecolor{CadetBlue3}{rgb}{0.478,0.773,0.804}
\definecolor{CadetBlue4}{rgb}{0.325,0.525,0.545}
\definecolor{turquoise1}{rgb}{0.000,0.961,1.000}
\definecolor{turquoise2}{rgb}{0.000,0.898,0.933}
\definecolor{turquoise3}{rgb}{0.000,0.773,0.804}
\definecolor{turquoise4}{rgb}{0.000,0.525,0.545}
\definecolor{cyan1}{rgb}{0.000,1.000,1.000}
\definecolor{cyan2}{rgb}{0.000,0.933,0.933}
\definecolor{cyan3}{rgb}{0.000,0.804,0.804}
\definecolor{cyan4}{rgb}{0.000,0.545,0.545}
\definecolor{DarkSlateGray1}{rgb}{0.592,1.000,1.000}
\definecolor{DarkSlateGray2}{rgb}{0.553,0.933,0.933}
\definecolor{DarkSlateGray3}{rgb}{0.475,0.804,0.804}
\definecolor{DarkSlateGray4}{rgb}{0.322,0.545,0.545}
\definecolor{aquamarine1}{rgb}{0.498,1.000,0.831}
\definecolor{aquamarine2}{rgb}{0.463,0.933,0.776}
\definecolor{aquamarine3}{rgb}{0.400,0.804,0.667}
\definecolor{aquamarine4}{rgb}{0.271,0.545,0.455}
\definecolor{DarkSeaGreen1}{rgb}{0.757,1.000,0.757}
\definecolor{DarkSeaGreen2}{rgb}{0.706,0.933,0.706}
\definecolor{DarkSeaGreen3}{rgb}{0.608,0.804,0.608}
\definecolor{DarkSeaGreen4}{rgb}{0.412,0.545,0.412}
\definecolor{SeaGreen1}{rgb}{0.329,1.000,0.624}
\definecolor{SeaGreen2}{rgb}{0.306,0.933,0.580}
\definecolor{SeaGreen3}{rgb}{0.263,0.804,0.502}
\definecolor{SeaGreen4}{rgb}{0.180,0.545,0.341}
\definecolor{PaleGreen1}{rgb}{0.604,1.000,0.604}
\definecolor{PaleGreen2}{rgb}{0.565,0.933,0.565}
\definecolor{PaleGreen3}{rgb}{0.486,0.804,0.486}
\definecolor{PaleGreen4}{rgb}{0.329,0.545,0.329}
\definecolor{SpringGreen1}{rgb}{0.000,1.000,0.498}
\definecolor{SpringGreen2}{rgb}{0.000,0.933,0.463}
\definecolor{SpringGreen3}{rgb}{0.000,0.804,0.400}
\definecolor{SpringGreen4}{rgb}{0.000,0.545,0.271}
\definecolor{green1}{rgb}{0.000,1.000,0.000}
\definecolor{green2}{rgb}{0.000,0.933,0.000}
\definecolor{green3}{rgb}{0.000,0.804,0.000}
\definecolor{green4}{rgb}{0.000,0.545,0.000}
\definecolor{chartreuse1}{rgb}{0.498,1.000,0.000}
\definecolor{chartreuse2}{rgb}{0.463,0.933,0.000}
\definecolor{chartreuse3}{rgb}{0.400,0.804,0.000}
\definecolor{chartreuse4}{rgb}{0.271,0.545,0.000}
\definecolor{OliveDrab1}{rgb}{0.753,1.000,0.243}
\definecolor{OliveDrab2}{rgb}{0.702,0.933,0.227}
\definecolor{OliveDrab3}{rgb}{0.604,0.804,0.196}
\definecolor{OliveDrab4}{rgb}{0.412,0.545,0.133}
\definecolor{DarkOliveGreen1}{rgb}{0.792,1.000,0.439}
\definecolor{DarkOliveGreen2}{rgb}{0.737,0.933,0.408}
\definecolor{DarkOliveGreen3}{rgb}{0.635,0.804,0.353}
\definecolor{DarkOliveGreen4}{rgb}{0.431,0.545,0.239}
\definecolor{khaki1}{rgb}{1.000,0.965,0.561}
\definecolor{khaki2}{rgb}{0.933,0.902,0.522}
\definecolor{khaki3}{rgb}{0.804,0.776,0.451}
\definecolor{khaki4}{rgb}{0.545,0.525,0.306}
\definecolor{LightGoldenrod1}{rgb}{1.000,0.925,0.545}
\definecolor{LightGoldenrod2}{rgb}{0.933,0.863,0.510}
\definecolor{LightGoldenrod3}{rgb}{0.804,0.745,0.439}
\definecolor{LightGoldenrod4}{rgb}{0.545,0.506,0.298}
\definecolor{LightYellow1}{rgb}{1.000,1.000,0.878}
\definecolor{LightYellow2}{rgb}{0.933,0.933,0.820}
\definecolor{LightYellow3}{rgb}{0.804,0.804,0.706}
\definecolor{LightYellow4}{rgb}{0.545,0.545,0.478}
\definecolor{yellow1}{rgb}{1.000,1.000,0.000}
\definecolor{yellow2}{rgb}{0.933,0.933,0.000}
\definecolor{yellow3}{rgb}{0.804,0.804,0.000}
\definecolor{yellow4}{rgb}{0.545,0.545,0.000}
\definecolor{gold1}{rgb}{1.000,0.843,0.000}
\definecolor{gold2}{rgb}{0.933,0.788,0.000}
\definecolor{gold3}{rgb}{0.804,0.678,0.000}
\definecolor{gold4}{rgb}{0.545,0.459,0.000}
\definecolor{goldenrod1}{rgb}{1.000,0.757,0.145}
\definecolor{goldenrod2}{rgb}{0.933,0.706,0.133}
\definecolor{goldenrod3}{rgb}{0.804,0.608,0.114}
\definecolor{goldenrod4}{rgb}{0.545,0.412,0.078}
\definecolor{DarkGoldenrod1}{rgb}{1.000,0.725,0.059}
\definecolor{DarkGoldenrod2}{rgb}{0.933,0.678,0.055}
\definecolor{DarkGoldenrod3}{rgb}{0.804,0.584,0.047}
\definecolor{DarkGoldenrod4}{rgb}{0.545,0.396,0.031}
\definecolor{RosyBrown1}{rgb}{1.000,0.757,0.757}
\definecolor{RosyBrown2}{rgb}{0.933,0.706,0.706}
\definecolor{RosyBrown3}{rgb}{0.804,0.608,0.608}
\definecolor{RosyBrown4}{rgb}{0.545,0.412,0.412}
\definecolor{IndianRed1}{rgb}{1.000,0.416,0.416}
\definecolor{IndianRed2}{rgb}{0.933,0.388,0.388}
\definecolor{IndianRed3}{rgb}{0.804,0.333,0.333}
\definecolor{IndianRed4}{rgb}{0.545,0.227,0.227}
\definecolor{sienna1}{rgb}{1.000,0.510,0.278}
\definecolor{sienna2}{rgb}{0.933,0.475,0.259}
\definecolor{sienna3}{rgb}{0.804,0.408,0.224}
\definecolor{sienna4}{rgb}{0.545,0.278,0.149}
\definecolor{burlywood1}{rgb}{1.000,0.827,0.608}
\definecolor{burlywood2}{rgb}{0.933,0.773,0.569}
\definecolor{burlywood3}{rgb}{0.804,0.667,0.490}
\definecolor{burlywood4}{rgb}{0.545,0.451,0.333}
\definecolor{wheat1}{rgb}{1.000,0.906,0.729}
\definecolor{wheat2}{rgb}{0.933,0.847,0.682}
\definecolor{wheat3}{rgb}{0.804,0.729,0.588}
\definecolor{wheat4}{rgb}{0.545,0.494,0.400}
\definecolor{tan1}{rgb}{1.000,0.647,0.310}
\definecolor{tan2}{rgb}{0.933,0.604,0.286}
\definecolor{tan3}{rgb}{0.804,0.522,0.247}
\definecolor{tan4}{rgb}{0.545,0.353,0.169}
\definecolor{chocolate1}{rgb}{1.000,0.498,0.141}
\definecolor{chocolate2}{rgb}{0.933,0.463,0.129}
\definecolor{chocolate3}{rgb}{0.804,0.400,0.114}
\definecolor{chocolate4}{rgb}{0.545,0.271,0.075}
\definecolor{firebrick1}{rgb}{1.000,0.188,0.188}
\definecolor{firebrick2}{rgb}{0.933,0.173,0.173}
\definecolor{firebrick3}{rgb}{0.804,0.149,0.149}
\definecolor{firebrick4}{rgb}{0.545,0.102,0.102}
\definecolor{brown1}{rgb}{1.000,0.251,0.251}
\definecolor{brown2}{rgb}{0.933,0.231,0.231}
\definecolor{brown3}{rgb}{0.804,0.200,0.200}
\definecolor{brown4}{rgb}{0.545,0.137,0.137}
\definecolor{salmon1}{rgb}{1.000,0.549,0.412}
\definecolor{salmon2}{rgb}{0.933,0.510,0.384}
\definecolor{salmon3}{rgb}{0.804,0.439,0.329}
\definecolor{salmon4}{rgb}{0.545,0.298,0.224}
\definecolor{LightSalmon1}{rgb}{1.000,0.627,0.478}
\definecolor{LightSalmon2}{rgb}{0.933,0.584,0.447}
\definecolor{LightSalmon3}{rgb}{0.804,0.506,0.384}
\definecolor{LightSalmon4}{rgb}{0.545,0.341,0.259}
\definecolor{orange1}{rgb}{1.000,0.647,0.000}
\definecolor{orange2}{rgb}{0.933,0.604,0.000}
\definecolor{orange3}{rgb}{0.804,0.522,0.000}
\definecolor{orange4}{rgb}{0.545,0.353,0.000}
\definecolor{DarkOrange1}{rgb}{1.000,0.498,0.000}
\definecolor{DarkOrange2}{rgb}{0.933,0.463,0.000}
\definecolor{DarkOrange3}{rgb}{0.804,0.400,0.000}
\definecolor{DarkOrange4}{rgb}{0.545,0.271,0.000}
\definecolor{coral1}{rgb}{1.000,0.447,0.337}
\definecolor{coral2}{rgb}{0.933,0.416,0.314}
\definecolor{coral3}{rgb}{0.804,0.357,0.271}
\definecolor{coral4}{rgb}{0.545,0.243,0.184}
\definecolor{tomato1}{rgb}{1.000,0.388,0.278}
\definecolor{tomato2}{rgb}{0.933,0.361,0.259}
\definecolor{tomato3}{rgb}{0.804,0.310,0.224}
\definecolor{tomato4}{rgb}{0.545,0.212,0.149}
\definecolor{OrangeRed1}{rgb}{1.000,0.271,0.000}
\definecolor{OrangeRed2}{rgb}{0.933,0.251,0.000}
\definecolor{OrangeRed3}{rgb}{0.804,0.216,0.000}
\definecolor{OrangeRed4}{rgb}{0.545,0.145,0.000}
\definecolor{red1}{rgb}{1.000,0.000,0.000}
\definecolor{red2}{rgb}{0.933,0.000,0.000}
\definecolor{red3}{rgb}{0.804,0.000,0.000}
\definecolor{red4}{rgb}{0.545,0.000,0.000}
\definecolor{DeepPink1}{rgb}{1.000,0.078,0.576}
\definecolor{DeepPink2}{rgb}{0.933,0.071,0.537}
\definecolor{DeepPink3}{rgb}{0.804,0.063,0.463}
\definecolor{DeepPink4}{rgb}{0.545,0.039,0.314}
\definecolor{HotPink1}{rgb}{1.000,0.431,0.706}
\definecolor{HotPink2}{rgb}{0.933,0.416,0.655}
\definecolor{HotPink3}{rgb}{0.804,0.376,0.565}
\definecolor{HotPink4}{rgb}{0.545,0.227,0.384}
\definecolor{pink1}{rgb}{1.000,0.710,0.773}
\definecolor{pink2}{rgb}{0.933,0.663,0.722}
\definecolor{pink3}{rgb}{0.804,0.569,0.620}
\definecolor{pink4}{rgb}{0.545,0.388,0.424}
\definecolor{LightPink1}{rgb}{1.000,0.682,0.725}
\definecolor{LightPink2}{rgb}{0.933,0.635,0.678}
\definecolor{LightPink3}{rgb}{0.804,0.549,0.584}
\definecolor{LightPink4}{rgb}{0.545,0.373,0.396}
\definecolor{PaleVioletRed1}{rgb}{1.000,0.510,0.671}
\definecolor{PaleVioletRed2}{rgb}{0.933,0.475,0.624}
\definecolor{PaleVioletRed3}{rgb}{0.804,0.408,0.537}
\definecolor{PaleVioletRed4}{rgb}{0.545,0.278,0.365}
\definecolor{maroon1}{rgb}{1.000,0.204,0.702}
\definecolor{maroon2}{rgb}{0.933,0.188,0.655}
\definecolor{maroon3}{rgb}{0.804,0.161,0.565}
\definecolor{maroon4}{rgb}{0.545,0.110,0.384}
\definecolor{VioletRed1}{rgb}{1.000,0.243,0.588}
\definecolor{VioletRed2}{rgb}{0.933,0.227,0.549}
\definecolor{VioletRed3}{rgb}{0.804,0.196,0.471}
\definecolor{VioletRed4}{rgb}{0.545,0.133,0.322}
\definecolor{magenta1}{rgb}{1.000,0.000,1.000}
\definecolor{magenta2}{rgb}{0.933,0.000,0.933}
\definecolor{magenta3}{rgb}{0.804,0.000,0.804}
\definecolor{magenta4}{rgb}{0.545,0.000,0.545}
\definecolor{orchid1}{rgb}{1.000,0.514,0.980}
\definecolor{orchid2}{rgb}{0.933,0.478,0.914}
\definecolor{orchid3}{rgb}{0.804,0.412,0.788}
\definecolor{orchid4}{rgb}{0.545,0.278,0.537}
\definecolor{plum1}{rgb}{1.000,0.733,1.000}
\definecolor{plum2}{rgb}{0.933,0.682,0.933}
\definecolor{plum3}{rgb}{0.804,0.588,0.804}
\definecolor{plum4}{rgb}{0.545,0.400,0.545}
\definecolor{MediumOrchid1}{rgb}{0.878,0.400,1.000}
\definecolor{MediumOrchid2}{rgb}{0.820,0.373,0.933}
\definecolor{MediumOrchid3}{rgb}{0.706,0.322,0.804}
\definecolor{MediumOrchid4}{rgb}{0.478,0.216,0.545}
\definecolor{DarkOrchid1}{rgb}{0.749,0.243,1.000}
\definecolor{DarkOrchid2}{rgb}{0.698,0.227,0.933}
\definecolor{DarkOrchid3}{rgb}{0.604,0.196,0.804}
\definecolor{DarkOrchid4}{rgb}{0.408,0.133,0.545}
\definecolor{purple1}{rgb}{0.608,0.188,1.000}
\definecolor{purple2}{rgb}{0.569,0.173,0.933}
\definecolor{purple3}{rgb}{0.490,0.149,0.804}
\definecolor{purple4}{rgb}{0.333,0.102,0.545}
\definecolor{MediumPurple1}{rgb}{0.671,0.510,1.000}
\definecolor{MediumPurple2}{rgb}{0.624,0.475,0.933}
\definecolor{MediumPurple3}{rgb}{0.537,0.408,0.804}
\definecolor{MediumPurple4}{rgb}{0.365,0.278,0.545}
\definecolor{thistle1}{rgb}{1.000,0.882,1.000}
\definecolor{thistle2}{rgb}{0.933,0.824,0.933}
\definecolor{thistle3}{rgb}{0.804,0.710,0.804}
\definecolor{thistle4}{rgb}{0.545,0.482,0.545}
\definecolor{gray5}{rgb}{0.051,0.051,0.051}
\definecolor{gray10}{rgb}{0.102,0.102,0.102}
\definecolor{gray15}{rgb}{0.149,0.149,0.149}
\definecolor{gray20}{rgb}{0.200,0.200,0.200}
\definecolor{gray25}{rgb}{0.251,0.251,0.251}
\definecolor{gray30}{rgb}{0.302,0.302,0.302}
\definecolor{gray35}{rgb}{0.349,0.349,0.349}
\definecolor{gray40}{rgb}{0.400,0.400,0.400}
\definecolor{gray45}{rgb}{0.451,0.451,0.451}
\definecolor{gray50}{rgb}{0.498,0.498,0.498}
\definecolor{gray55}{rgb}{0.549,0.549,0.549}
\definecolor{gray60}{rgb}{0.600,0.600,0.600}
\definecolor{gray65}{rgb}{0.651,0.651,0.651}
\definecolor{gray70}{rgb}{0.702,0.702,0.702}
\definecolor{gray75}{rgb}{0.749,0.749,0.749}
\definecolor{gray80}{rgb}{0.800,0.800,0.800}
\definecolor{gray85}{rgb}{0.851,0.851,0.851}
\definecolor{gray90}{rgb}{0.898,0.898,0.898}
\definecolor{gray95}{rgb}{0.949,0.949,0.949}
\definecolor{gray100}{rgb}{1.000,1.000,1.000}
\definecolor{DarkGray}{rgb}{0.663,0.663,0.663}
\definecolor{DarkBlue}{rgb}{0.000,0.000,0.545}
\definecolor{DarkCyan}{rgb}{0.000,0.545,0.545}
\definecolor{DarkMagenta}{rgb}{0.545,0.000,0.545}
\definecolor{DarkRed}{rgb}{0.545,0.000,0.000}
\definecolor{LightGreen}{rgb}{0.565,0.933,0.565}


==> header.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%2345678901234567890123456789012345678901234567890123456789012345678901234567890
%        1         2         3         4         5         6         7         8

  % Comment this line out
                                                          % if you need a4paper
%\documentclass[a4paper, 10pt, conference]{ieeeconf}      % Use this line for a4
                                                          % paper

\IEEEoverridecommandlockouts                              % This command is only
                                                          % needed if you want to
                                                          % use the \thanks command
\overrideIEEEmargins
% See the \addtolength command later in the file to balance the column lengths

\usepackage{amsmath}
\usepackage{bm}	
\usepackage{graphicx}

\newtheorem{Assumption}{Assumption}
\newtheorem{Theorem}{Theorem}
\newtheorem{Condition}{Condition}
\newtheorem{Corollary}{Corollary}
\newtheorem{Definition}{Definition}
\newtheorem{Lemma}{Lemma}
%\newtheorem*{Proof*}{Proof}
%\newtheorem{Proof}{Proof}
\newtheorem{Proposition}{Proposition}
\newtheorem{Result}{Result}
\newtheorem{Remark}{Remark}

==> introduction.tex <==
\section{Introduction}

%background: electronic toll collection
Vehicle-to-infrastructure (V2I) communications are increasingly applied to modern highways in order to improve efficiency, reliability, and safety \cite{varaiya93}.
An important application of the V2I communications is multi-priority lane management operations for heterogeneous traffic.
For example, electronic toll collection is enabled by onboard device and road side units (RSU) that exchange data \cite{papadimitratos09}.
Other examples of lane management operations include high-occupancy vehicle (HOV) and high occupancy tolled (HOT) lanes \cite{kurzhanskiy15}, and, as a proposed operation, dedicated lanes for vehicle platoons \cite{bergenhem12,jin18hscc}.


%This model is suitable for operational situations in which various traffic classes need to be segmented on different lanes, such as tolled lanes \cite{papadimitratos09}, heavy/high-occupancy vehicle access \cite{kurzhanskiy15}, or platooning operations \cite{bergenhem12}.
%In addition, we consider that the facility is equipped with the cyber infrastructure (e.g. road-side units, RSU) that is capable of receiving messages from the individual vehicles and monitor the traffic as it gets segmented into different lanes. 
%Such a capability is made possible by the presence of onborad units (OBU) in modern vehicle systems that communicate (via e.g. DSRC/RFID/GPS) necessary information to the RSU.
%Examples of information that these messages carry include vehicle identifiers, vehicle class, toll debit information, safety-related information (e.g. speed/acceleration), etc.


%background: misbehavior
We consider V2I communications enabled by the cyber infrastructure (e.g. road-side units, RSU) that receives messages from the individual vehicles for authentication purposes and monitors the traffic as it gets segmented into different lanes. 
Naturally, this capability assumes the presence of an onboard unit (OBU) on individual vehicles that access the highway system.
Technologies commonly used V2I communications include Dedicated Short Range Communications (DSRC), Radio Frequency Identification (RFID), and Global Positioning System (GPS) \cite{papadimitratos09,depalma11}.
Upon arrival to the system, each vehicle (i.e. its OBU) sends a message to the RSU through one or more channels; this message can include information such as vehicle identifier, vehicle class, toll debit information, safety-related information (e.g. speed/acceleration), etc.

All of these technologies to some extent rely on the information/data reported by the vehicles.
%Therefore, a vehicle is capable of obtaining illegal access to priority lanes by manipulating the information reported to the road-side units, if such misbehavior brings the driver benefits such as reduced travel time.
%For DSRC, a vehicle may misreport its identity information \cite{petit15}.
%For RFID, a vehicle may copy the identity number of another vehicle and thus induce the toll on others \cite{lawson08}.
%GPS-based communications also have similar vulnerabilities \cite{hubaux04}.
Motivated by previously reported vulnerabilities in the V2I communications technology \cite{hubaux04,lawson08,petit15}, we consider that individual travelers may manipulate the message, albeit at a cost, so that the RSU receives false information and incorrectly authorizes such agents.
In this paper, we focus on the incentive of agents to misreport their vehicle identity information to gain illegal access to the lanes dedicated to other traffic classes. Such misbehavior can result in losses such as lost toll revenue, operational inefficiencies, or even safety risks; hence, it should be inspected by the system operator.

%background: inspection
Due to the large number of devices involved in V2I communications, full prevention of misbehavior is neither technologically nor economically feasible.
However, there are several inspection schemes in response to potential misbehaviors.
Within V2I communications, internal learning-based verification algorithms may detect
Beyond V2I communications, the system operator may have access to other sources of information for cross verification \cite{}.
For example, Automated Number Plate Recognition (ANPR) is also a commonly used vehicle identification technology \cite{depalma11}.
If a highway is equipped with both V2I communications and ANPR, then the system operator may have the capability of cross-checking data retrieved via both technologies.
Another example is police patrol with random inspection of misbehavior \cite{borndorfer13}.
Note that both inspection schemes may require additional investment in infrastructure or labor, and may induce additional congestion.

%our contributions
In this article, we develop a framework for quantitative estimate of the incentive for a class of misbehavior and design of effective and economically efficient inspection schemes.
We also account for the main tradeoff faced by the system operator in inspecting the agents for misbehavior.
For potential misbehaving vehicles, we evaluate the benefit (travel time reduction) resulting from misbehavior, and study the probability of misbehavior of a strategic driver that is aware of the cost of conducting misbehavior (technological investment and potential fine).
For the system operator, we study the optimal inspection strategy in terms of inspection probability/rate and the fine for misbehavior.

%literature: toll evasion
%\textcolor{violet}{
%Some authors have used game-theoretic approaches to study misbehavior in conventional transportation systems.
%Yin et al. \cite{yin12} studied randomized patrol strategies for fare inspection in public transportation based on a Stackelberg formulation.
%Bornd\"ofer et al. \cite{borndorfer13} considered optimal inspector allocation in highway networks facing misbehaving travelers that may strategically choose their routes.
%However, limited results are available on misbehavior in smart transportation systems with cyber-physical vulnerabilities.
%To address this challenge, we develop a framework that explicitly captures key features of V2I-based highway operations.
%}

\begin{figure}[H]
\centering
\includegraphics[width=0.5\textwidth]{./figures/toll_lanes}
\caption{An automated highway with V2I-based lane management operations.}
\label{toll_lanes}
\end{figure}

%our physical
Our analysis considers an automated highway section with a downstream bottleneck (Sec. \ref{sec_physical}).
The highway section has a set of high-priority (e.g. tolled or HOV) lanes and a set of low-priority (e.g. general-purpose) lanes; see Fig.~\ref{toll_lanes}.
We consider the two sets of lanes as two parallel servers.
The highway faces two types of vehicles: high-priority vehicles and low-priority vehicles.
Upon arrival, each vehicles reports its types to the system operator via V2I communications.
Then, the system operator authorizes the vehicle access to the high-priority server if the vehicle is reportedly a high-priority-type vehicle.
Every lane has a travel cost that increases with the number of vehicles taking this lane.
Our formulation is compatible with a broad class of travel cost functions with such monotonicity.
While we do not specialize our model to capture losses such as lost toll revenue or safety risk, we do capture the key contributing factor: the congestion externality induced by misbehaving agents on the other travelers.
%We model the highway bottleneck in Fig.~\ref{toll_lanes} as two parallel $M/M/1$ queuing systems.
%However, we emphasize that our framework is compatible with a broad class of queuing/fluid models for various transportation systems \cite{newell13,jin18hscc}.

%our cyber model

To study the interaction between misbehaving vehicles and the system operator, we consider a signaling game formulation (Sec. \ref{sec_misbehavior}). 
Signaling game is a natural choice for our purpose, since we particularly focus on vehicles strategically abusing the V2I communications.
The vehicles are modeled as a set of non-atomic agents, and the system operator is considered as the defender. Each agent privately knows its type, i.e. high- or low-priority.
In addition, each agent sends a signal of its type to the system operator (defender), which may not match its true type. 
We say that the agent misbehaves if it sends a signal different from its true type, and thus uses a server that does not match its type.
For a low-priority agent, conducting a misbehavior induces a strictly positive technological cost.
For the sake of generality, we also consider a high-priority vehicle sending a low-priority signal as ``misbehaving'' (the technological cost for such a ``misbehavior'' can be made zero.)
This construction allows us to consider the possible incentive of a high-priority agent to switch to the low-priority server.
The defender observes the signal that an agent sends but does not know the agent's true type. 
The defender then forms a belief about the fraction of agents who misbehave, and determines the inspection rate on each server. If an agent misbehaves, and is inspected, then the misbehavior is detection. A fine is charged to the agent by the defender. 

The equilibrium concept that we use is the Perfect Bayesian Equilibrium (PBE), where the agents and the defender are sequentially rational, and the defender's belief is consistent with the prior distribution and the agents' strategy according to Bayes' rule. Our game is different from the classical signaling game (see \cite{spence1974market,fudenberg1991perfect,cho1987signaling,banks1987equilibrium}) in two aspects: (1) The agents are considered as non-atomic players; (2) Both lanes are congested since the cost of each lane increases in the aggregate demand of agents on it. In fact, these two features make the equilibrium properties of our game different from those classical models. 

%our analysis approach
Based on the signaling game formulation, we are able to characterize the equilibrium behavior of agents and the system operator (Sec. \ref{sec_equilibrium}). Our analysis is based on a set of mild assumptions regarding the baseline scenario where no agent misbehaves (Assumptions (A1)). We show that in equilibrium (i) a high-priority agent never has the incentive to switch to the low-priority server (Proposition \ref{h_non_deviate}), and (ii) not every low-priority agent misbehaves (Proposition \ref{no_pool}). In general, there are two regimes based on the magnitude of misbehavior cost compared to the maximum misbehavior incentive, which is the travel cost difference on two servers when no agents misbehave: in the first regime, denoted by $\A$, the misbehavior cost is higher, and thus misbehavior is deterred, whereas in the second regime, denoted by $\B$, the misbehavior cost is lower, and thus the misbehavior rate is always positive in equilibrium. Furthermore, three sub-regimes exist in regime $\B$, where the defender chooses to inspect no agents, a fraction of agents and all agents, respectively (Theorem \ref{theorem_equilibrium}).
%In general, the misbehavior rate is non-increasing in the misbehavior cost, and non-decreasing in the inspection cost. The inspection rate is non-increasing in both the misbehavior cost and the inspection cost. 
%Our analysis also shows that the increase in fine can decrease the misbehavior rate, but is only effective when the misbehavior cost is medium or low.  % ($\Bone$) Given a high misbehavior cost or a high inspection cost, the misbehavior rate is low, and the defender does not inspect; ($\Btwo$) Given a low misbehavior cost and a medium inspection cost, the misbehavior rate is medium, and the defender inspects imperfectly; ($\Bthree$) Given a low misbehavior cost and a low inspection cost, the misbehavior rate is low, and the defender inspects perfectly .}

\textcolor{violet}{We also demonstrate practical implication from our analysis for cyber-physical security in smart highways (Sec. \ref{sec_implication}). For illustration purpose, we consider a specific setting of electronic toll collection (ETC). We show that given any misbehavior cost and inspection cost, as the fraction of agents who are willing to pay the toll increases, the misbehavior rate is lower and the inspection is less needed. Moreover, when the inspection cost is relatively high comparing to the misbehavior cost, fine is effective in decreasing the misbehavior rate, but does not deter misbehavior completely. 
Finally, if the fine is higher than the maximum misbehavior incentive, then the defender does not have to inspect every agent (i.e. the regime of complete inspection is empty).
}

%outline


==> physical_model_old.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Physical model for highway traffic} \label{sec_physical}
In this section, we discuss three physical models of highway traffic. In these models, two classes of traffic are given different priorities: The class of traffic with high priority is permitted to use the lane with lower travel time, whereas the class with low priority can only use the other lane with higher travel time. Travelers in the low priority class have incentive to sneak in the high priority lane by \textcolor{red}{to be filled in}. Therefore, the issue of misbehavior and how to inspect them naturally arise. 
\subsection{Toll system with ordinary traffic}\label{sec_toll}
\subsection{Mixed traffic with CAVs and ordinary traffic}\label{sec_mixed_traffic}
\subsection{Two classes of CAV traffic}\label{sec_two_classes}
%In this section, we introduce three physical models of highway traffic: 
%Consider a highway section with a downstream bottleneck. The capacity of the bottleneck is $U$. Both background traffic (ordinary vehicles) and platoons of connected/autonomous vehicles (CAV) use this link. The background traffic arrives continuously with deterministic arrival rate $a$. CAV forms platoons with exponentially distributed headways; the average headway is $1/\lambda$. The lengths of platoons are exponentially distributed with average $s/\mu$, where $s$ is the saturation rate of CAV platoons.
%
%The highway lanes are divided into two classes. The first class is the \emph{mixed lanes}, which both ordinary vehicles and platoons can use. Furthermore, ordinary vehicles do not enter these lanes if there is a platoon entering them. The second class is the \emph{ordinary lanes}, which ordinary vehicles can use but platoons cannot. For ease of presentation, we assume that each class of lanes has an aggregate capacity of $U/2$.
%
%We consider a simple route choice model that achieves the Wardrop equilibrium. 
%When no platoons are entering the highway, the background traffic flow is evenly distributed to both classes of lanes; otherwise, the aggregate traffic flow is evenly distributed:
%\begin{align*}
%&A_1(t)=\left\{\begin{array}{ll}
%\frac{a+s}{2}, & B(t)>0,\\
%\frac{a}{2}, & B(t)=0,
%\end{array}\right.
%\\
%&A_2(t)=\left\{\begin{array}{ll}
%\frac{a-s}{2}, & B(t)>0,\\
%\frac{a}{2}, & B(t)=0.
%\end{array}\right.
%\end{align*}
%Throughout this article, we assume that
%\begin{align*}
%a>s,
%\end{align*}
%which ensures non-negativity of $A_2(t)$.
%
%Since the background traffic is distributed according to the arrival process $B(t)$ of CAV platoons, how $B(t)$ evolves with time impacts the background traffic. Following the argument in \cite{jin18hscc}. we assume that (i) the inter-platoon headways are i.i.d. and exponentially distributed with the average $1/\lambda$, and (ii) the number of vehicles in platoons are also i.i.d. and exponentially distributed with the average $v/(\mu h)$, where $v$ is the \emph{free-flow speed} and $h$ is the \emph{intra-platoon spacing}.
%
%\section{Estimate of congestion externality due to misreporting}
%
%According to the misbehavior model, the highway dynamics switches between three modes.
%
%Although we are able to analytically compute the queue length associated with three modes, the expression is complex and does not enable tractable further analysis. To address this challenge, we consider a two-mode approximation of the three-mode system.
%
%Specifically, we approximate the superposition of two types of platoons with a single type with average length $p\nu+(1-p)\mu$.
%
%Let
%\begin{align*}
%&D=
%\left[\begin{array}{ccc}
%(a-u)/2& & \\
% & (a+s-u)/2 & \\
% & & 0 \end{array}\right],\\
%&Q=
%\left[\begin{array}{ccc}
%-\lambda & p\lambda & -1 \\
% \nu & -\nu & -1 \\
%\mu & 0 & -1\end{array}\right],\\
%&\hat Q=
%\left[\begin{array}{ccc}
%-\lambda & p\lambda & -1 \\
%p\nu+(1-p)\mu & -p\nu-(1-p)\mu & -1 \\
%p\nu+(1-p)\mu & 0 & -1\end{array}\right]
%\end{align*}
%
%\begin{Proposition}
%The approximation error is upper-bounded as follows:
%\begin{align*}
%\overline q-\hat q\le
%[0\; 0\; 1](\sum_{i=1}^2\beta_iD-Q)^{-1}
%\left[\begin{array}{c}1/\beta_1\\1/\beta_2\\0\end{array}\right]
%\end{align*}
%\end{Proposition}
%\begin{proof}
%The equation
%\begin{align*}
%\mathrm{det}(\beta D-Q)=0
%\end{align*}
%has three solutions $\beta_1,\beta_2,\beta_3$, where $\beta_1,\beta_2<0$, $\beta_3=0$. Let
%\begin{align*}
%\phi_i=
%e_3^T
%(\beta_iD-Q)^{-1},
%\quad i=1,2.
%\end{align*}
%
%Define the matrix
%\begin{align*}
%\Phi:=
%\left[\begin{array}{c}
%\phi_1\\
%\phi_2\\
%e_3^T\end{array}\right]
%=e_1e_3^T(\beta_1D-Q)^{-1}+e_2e_3^T(\beta_2D-Q)^{-1}+e_3e_3^T.
%\end{align*}
%Then we have
%\begin{align*}
%\overline q
%=e_3^T\Phi^{-1}\left[\begin{array}{c}1/\beta_1\\1/\beta_2\\0\end{array}\right].
%\end{align*}
%
%Hence, the maximum error is given by
%\begin{align*}
%\hat q-\overline q
%\end{align*}
%
%\end{proof}
